Automated Action Model Acquisition from Narrative Texts

Action models, which take the form of precondition/effect axioms, facilitate causal and motivational connections between actions for AI agents. Action model acquisition has been identified as a bottleneck in the application of planning technology, especially within narrative planning. Acquiring action models from narrative texts in an automated way is essential, but challenging because of the inherent complexities of such texts. We present NaRuto, a system that extracts structured events from narrative text and subsequently generates planning-language-style action models based on predictions of commonsense event relations, as well as textual contradictions and similarities, in an unsupervised manner. Experimental results in classical narrative planning domains show that NaRuto can generate action models of significantly better quality than existing fully automated methods, and even on par with those of semi-automated methods.

==> table-american-west-story.tex <==
\begin{tabular}{llll}
    \toprule
    \bfseries GT                   &     \bfseries Semi-auto \cite{hayton:etal:KEPS:2017}    &     \bfseries Semi-auto \cite{feng:ieee:2020}     &     \bfseries Our Approach                            \\ 
    \midrule
    \Extracted{die}                &     \checkmark \Extracted{died}                         &     \checkmark \Extracted{died}                   &     \checkmark \Extracted{die}               \\
    \Extracted{heal}               &     \checkmark \Extracted{healed}                       &     \checkmark \Extracted{healed}                 &     \checkmark \Extracted{heal}              \\ 
    \Extracted{shoot}              &     \checkmark \Extracted{shot}                         &     \checkmark \Extracted{shot}                   &     \checkmark \Extracted{shoot}             \\
    \Extracted{steal}              &     \checkmark \Extracted{stole}                        &     \checkmark \Extracted{stole}                  &     \checkmark \Extracted{steal}             \\
    \Extracted{snakebite}          &     \checkmark \Extracted{bitten}                       &     \HalfExtracted \Extracted{got}                &     \checkmark \Extracted{get bitten}        \\
                                   &     \HalfExtracted \Extracted{intended}                 &     \checkmark \Extracted{intended to heal}       &     \checkmark \Extracted{intend to heal}    \\
                                   &                                                         &     \checkmark \Extracted{intended to shoot}      &     \checkmark \Extracted{intend to shoot}   \\
                                   &                                                         &     \Missing \Extracted{using}                    &     \Missing \Extracted{use}                 \\
                                   &                                                         &     \Missing \Extracted{angered}                  &     \Missing \Extracted{anger}               \\
    \bottomrule
\end{tabular}

==> table-evaluation.tex <==
\begin{tabular}{llccc} 
&                                                 & \textbf{Sco. $\uparrow$}      &  \textbf{Agg. $\uparrow$}         & \textbf{Disagg. $\downarrow$} \\
\toprule
\multirow{9}{*}{\textbf{West}}
& GT~\cite{ware2014plan}                          & \multirow{1}{*}{4.34            }                               & \multirow{1}{*}{82.7\%            }                                 & \multirow{1}{*}{10.7\%            } \\ \cmidrule{2-5}
& StoryFramer~\cite{hayton:etal:KEPS:2017}        & \multirow{2}{*}{\underline{3.26}}                               & \multirow{2}{*}{42.5\%            }                                 & \multirow{2}{*}{\underline{26.3\%}} \\
& (Semi-auto)                                     &                                                                 &                                                                     &                                     \\ \cmidrule{2-5}
& H2020~\cite{hayton:etal:AAAI:2020}              & \multirow{2}{*}{2.54            }                               & \multirow{2}{*}{17.7\%            }                                 & \multirow{2}{*}{41.2\%            } \\
& (Auto)                                          &                                                                 &                                                                     &                                     \\ \cmidrule{2-5}
& NARuto (G)                                      & \multirow{1}{*}{2.98            }                               & \multirow{1}{*}{\underline{43.0\%}}                                 & \multirow{1}{*}{39.3\%            } \\ \cmidrule{2-5}
& NARuto (L)                                      & \multirow{1}{*}{\textbf{3.57}   }                               & \multirow{1}{*}{\textbf{60.8\%}   }                                 & \multirow{1}{*}{\textbf{25.3\%}   } \\ \toprule
\multirow[c]{9}{*}{\textbf{Aladdin}}
& GT~\cite{ware2014plan}                          & 4.84                                                            & 97.3\%                                                              & 1.2\%                               \\ \cmidrule{2-5}
& StoryFramer~\cite{hayton:etal:KEPS:2017}        & \multirow{2}{*}{\textbf{4.04}   }                               & \multirow{2}{*}{\textbf{74.8\%}   }                                 & \multirow{2}{*}{\textbf{17.3\%}   } \\
& (Semi-auto)                                     &                                                                 &                                                                     &                                     \\ \cmidrule{2-5}
& H2020~\cite{hayton:etal:AAAI:2020}              & \multirow{2}{*}{2.81            }                               & \multirow{2}{*}{38.2\%            }                                 & \multirow{2}{*}{48.8\%            } \\
& (Auto)                                          &                                                                 &                                                                     &                                     \\ \cmidrule{2-5}
& NARuto (G)                                      & \multirow{1}{*}{3.03            }                               & \multirow{1}{*}{41.0\%            }                                 & \multirow{1}{*}{38.3\%            } \\ \cmidrule{2-5}
& NARuto (L)                                      & \multirow{1}{*}{\underline{3.34}}                               & \multirow{1}{*}{\underline{52.0\%}}                                 & \multirow{1}{*}{\underline{29.5\%}} \\
\bottomrule


\end{tabular}
